Phenomenological quark-hadron equations of state with first-order phase transitions for astrophysical applications

In the current work an equation of state model with a first-order phase transition for astrophysical applications is presented. The model is based on a two-phase approach for quark-hadron phase transitions, which leads by construction to a first-order phase transition. The resulting model has already been successfully used in several astrophysical applications, such as cold neutron stars, core-collapse supernova explosions and binary neutron star mergers. Main goal of this work is to present the details of the model, discuss certain features and eventually publish it in a tabulated form for further use.

==> niels-glossary.tex <==
\newabbreviation[longplural={equations of state},description={Equations of state relate thermodynamic quantities, which describe the state of matter.}]{eos}{EoS}{equation of state}
%~ \newabbreviation[longplural={degrees of freedom}]{dof}{dof}{degree of freedom}
\newabbreviation[shortplural={HIC}]{hic}{HIC}{heavy-ion collisions}
\newabbreviation[description={Nuclotron-based Ion Collider fAcility in Dubna, Russia}]{nica}{NICA}{Nuclotron-based Ion Collider fAcility}
\newabbreviation{qmd}{QMD}{quantum molecular dynamic}
\newabbreviation{urqmd}{UrQMD}{ultra-relativistic quantum molecular dynamic}
\newabbreviation{amd}{AMD}{antisymmetrized molecular dynamics}
\newabbreviation{rdf}{RDF}{relativistic density functional}
\newabbreviation{rmf}{RMF}{relativistic mean field}
\newabbreviation{sfm}{SFM}{string-flip model}
\newabbreviation{qcd}{QCD}{quantum chromodynamics}
\newabbreviation{qgp}{QGP}{quark-gluon plasma}
\newabbreviation{cep}{CEP}{critical endpoint}
\newabbreviation{njl}{NJL}{Nambu-Jona-Lasinio}
	\newabbreviation[parent=njl,description={}]{hnjl}{hNJL}{higher order \glsentryshort{njl}}
	\newabbreviation[parent=njl,description={}]{hnjlb}{hNJLb}{higher order \glsentryshort{njl} with bag constant}
	\newabbreviation[parent=njl,description={}]{pnjl}{PNJL}{Polyakov-loop \glsentrylong{njl}}
\newabbreviation{nse}{NSE}{nuclear statistical equilibrium}
%~ \newabbreviation{qs}{QS}{quantum statistical}
\newabbreviation{cve}{CVE}{cluster virial expansion}
%~ \newabbreviation{ns}{NS}{neutron star}
%~ \newabbreviation{pt}{PT}{phase transition}
%~ \newabbreviation{pns}{PNS}{proto-neutron star}
\newabbreviation{bnsm}{BNSM}{binary neutron star merger}
\newabbreviation{tov}{TOV}{Tolman--Oppenheimer--Volkoff}
\newabbreviation{gr}{GR}{general relativity}
\newabbreviation[longplural={core-collapse supernovae}]{ccsn}{CCSN}{core-collapse supernova}
\newabbreviation[description={Zero Age Main Sequence is the time when a star starts burning hydrogen and therefore joins the main sequence on the Hertzsprung-Russell diagram}]{zams}{ZAMS}{zero-age main sequence}
\newabbreviation{sb}{SB}{Stefan-Boltzmann}

\newabbreviation{n3lo}{N$^3$LO}{next-to-next-to-next-to-leading order}
\newabbreviation{ceft}{$\chi$EFT}{chiral effective field theory}
\newabbreviation{pqcd}{pQCD}{perturbative QCD}

\newglossaryentry{bu}{name={Beth-Uhlenbeck},description={}}
	\newglossaryentry{gbu}{name={generalized Beth-Uhlenbeck},parent=bu,description={}}
\newglossaryentry{cern}{name={CERN},description={European Organization for Nuclear Research in Geneva, Switzerland}}
\newglossaryentry{lhc}{name={LHC},description={Large Hadron Collider experiment at \gls{cern}}}
\newglossaryentry{alice}{name={ALICE},description={A Large Ion Collider Experiment}}
\newglossaryentry{rhic}{name={RHIC},description={Relativistic Heavy Ion Collider at the Brookhaven National Laboratory in Upton, USA}}
\newglossaryentry{fair}{name={FAIR},description={Facility for Antiproton and Ion Research at GSI in Darmstadt, Germany}}
\newglossaryentry{dd2all}{name={DD2(F)},description={Walecka-type hadron model with density dependent couplings}}
	\newglossaryentry{dd2}{name={DD2},parent=dd2all,description={}}
	\newglossaryentry{dd2f}{name={DD2F},parent=dd2all,description={}}
\newglossaryentry{theseus}{name={THESEUS},description={Three-fluid Hydrodynamics-based Event Simulator Extended by UrQMD final State interactions}}
\newglossaryentry{rhic:bes}{name={RHIC BES},parent=rhic,description={}}
\newglossaryentry{rhic:fxt}{name={RHIC FXT},parent=rhic,description={}}
\newglossaryentry{na61}{name={NA61},description={NA61}}
\newglossaryentry{lqcd}{name={Lattice QCD},description={lattice QCD}}
\newglossaryentry{nicer}{name={NICER}, description={Neutron Star Interior Composition Explorer \url{https://www.nasa.gov/nicer}}}


